SMG: A Shuffling Gradient-Based Method with Momentum

We combine two advanced ideas widely used in optimization for machine learning: shuffling strategy and momentum technique to develop a novel shuffling gradient-based method with momentum, coined Shuffling Momentum Gradient (SMG), for non-convex finite-sum optimization problems. While our method is inspired by momentum techniques, its update is fundamentally different from existing momentum-based methods. We establish state-of-the-art convergence rates of SMG for any shuffling strategy using either constant or diminishing learning rate under standard assumptions (i.e.$L$-smoothness and bounded variance). When the shuffling strategy is fixed, we develop another new algorithm that is similar to existing momentum methods, and prove the same convergence rates for this algorithm under the $L$-smoothness and bounded gradient assumptions. We demonstrate our algorithms via numerical simulations on standard datasets and compare them with existing shuffling methods. Our tests have shown encouraging performance of the new algorithms.

==> refs.tex <==
\begin{thebibliography}{42}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Abadi et al(2015)]{tensorflow2015-whitepaper}
M.~Abadi {\emph{et al}}.
\newblock {TensorFlow}: Large-scale machine learning on heterogeneous systems,
  2015.
\newblock URL \url{https://www.tensorflow.org/}.
\newblock Software available from tensorflow.org.

\bibitem[Bertsekas(2011)]{Bertsekas2011}
D. P. Bertsekas.
\newblock Incremental proximal methods for large scale convex optimization.
\newblock \emph{Math. Program.}, 129\penalty0 (2):\penalty0 163--195, 2011.

\bibitem[Bottou(2009)]{bottou2009curiously}
L.~Bottou.
\newblock Curiously fast convergence of some stochastic gradient descent
  algorithms.
\newblock 2009.

\bibitem[Bottou(2012)]{bottou2012stochastic}
L.~Bottou.
\newblock Stochastic gradient descent tricks.
\newblock In \emph{Neural networks: Tricks of the trade}, pages 421--436.
  Springer, 2012.

\bibitem[Bottou et~al.(2018)Bottou, Curtis, and Nocedal]{Bottou2018}
L.~Bottou, F.~E. Curtis, and J.~Nocedal.
\newblock {O}ptimization {M}ethods for {L}arge-{S}cale {M}achine {L}earning.
\newblock \emph{SIAM Rev.}, 60\penalty0 (2):\penalty0 223--311, 2018.

\bibitem[Chang and Lin(2011)]{LIBSVM}
Chih-Chung Chang and Chih-Jen Lin.
\newblock {LIBSVM}: A library for support vector machines.
\newblock \emph{ACM Transactions on Intelligent Systems and Technology},
  2:\penalty0 27:1--27:27, 2011.
\newblock Software available at \url{http://www.csie.ntu.edu.tw/~cjlin/libsvm}.

\bibitem[Chen et~al.(2018)Chen, Liu, Sun, and Hong]{chen2018convergence}
X.~Chen, S.~Liu, R.~Sun, and M.~Hong.
\newblock On the convergence of a class of adam-type algorithms for non-convex
  optimization.
\newblock \emph{ICLR}, 2018.

\bibitem[Defazio et~al.(2014)Defazio, Bach, and Lacoste-Julien]{SAGA}
Aaron Defazio, Francis Bach, and Simon Lacoste-Julien.
\newblock Saga: A fast incremental gradient method with support for
  non-strongly convex composite objectives.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  1646--1654, 2014.

\bibitem[Dozat(2016)]{dozat2016incorporating}
T. Dozat.
\newblock Incorporating nesterov momentum into {ADAM}.
\newblock \emph{ICLR Workshop}, 1:\penalty0 2013–--2016, 2016.

\bibitem[Duchi et~al.(2011)Duchi, Hazan, and Singer]{AdaGrad}
John Duchi, Elad Hazan, and Yoram Singer.
\newblock Adaptive subgradient methods for online learning and stochastic
  optimization.
\newblock \emph{Journal of Machine Learning Research}, 12:\penalty0 2121--2159,
  2011.

\bibitem[Ghadimi and Lan(2013)]{ghadimi2013stochastic}
S.~Ghadimi and G.~Lan.
\newblock Stochastic first-and zeroth-order methods for nonconvex stochastic
  programming.
\newblock \emph{SIAM J. Optim.}, 23\penalty0 (4):\penalty0 2341--2368, 2013.

% \bibitem[G{\"u}rb{\"u}zbalaban et~al.(2015)G{\"u}rb{\"u}zbalaban, Ozdaglar, and
%   Parrilo]{gurbuzbalaban2015random}
% Mert G{\"u}rb{\"u}zbalaban, Asu Ozdaglar, and Pablo Parrilo.
% \newblock Why random reshuffling beats stochastic gradient descent.
% \newblock \emph{arXiv preprint arXiv:1510.08560}, 2015.

\bibitem[HaoChen and Sra(2018)]{haochen2018random}
Jeffery~Z HaoChen and Suvrit Sra.
\newblock Random shuffling beats sgd after finite epochs.
\newblock \emph{arXiv preprint arXiv:1806.10077}, 2018.

\bibitem[Johnson and Zhang(2013)]{SVRG}
Rie Johnson and Tong Zhang.
\newblock Accelerating stochastic gradient descent using predictive variance
  reduction.
\newblock In \emph{NIPS}, pages 315--323, 2013.

\bibitem[Kingma and Ba(2014)]{Kingma2014}
D.~P. Kingma and J.~Ba.
\newblock {ADAM}: {A} {M}ethod for {S}tochastic {O}ptimization.
\newblock \emph{Proceedings of the 3rd International Conference on Learning
  Representations (ICLR)}, abs/1412.6980, 2014.

\bibitem[Krizhevsky and Hinton(2009)]{CIFAR10}
Alex Krizhevsky and Geoffrey Hinton.
\newblock Learning multiple layers of features from tiny images.
\newblock Technical report, Citeseer, 2009.

\bibitem[LeCun et~al.(1998)LeCun, Bottou, Bengio, and Haffner]{MNIST}
Yann LeCun, L{\'e}on Bottou, Yoshua Bengio, and Patrick Haffner.
\newblock Gradient-based learning applied to document recognition.
\newblock \emph{Proceedings of the IEEE}, 86\penalty0 (11):\penalty0
  2278--2324, 1998.

\bibitem[Li et~al.(2020)Li, Zhuang, and Orabona]{li2020exponential}
L.~Li, Z.~Zhuang, and F.~Orabona.
\newblock Exponential step sizes for non-convex optimization.
\newblock \emph{arXiv preprint arXiv:2002.05273}, 2020.

\bibitem[Li et~al.(2019)Li, Zhu, So, and Lee]{li2019incremental}
X.~Li, Z.~Zhu, A.~So, and J.~D. Lee.
\newblock Incremental methods for weakly convex optimization.
\newblock \emph{arXiv preprint arXiv:1907.11687}, 2019.

\bibitem[Loshchilov and Hutter(2017)]{loshchilov10sgdr}
I.~Loshchilov and F.~Hutter.
\newblock {SGDR}: {S}tochastic gradient descent with warm restarts.
\newblock 10:\penalty0 1--16, 2017.

\bibitem[Loshchilov and Hutter(2016)]{loshchilov2016sgdr}
Ilya Loshchilov and Frank Hutter.
\newblock Sgdr: Stochastic gradient descent with warm restarts, 2016.

\bibitem[Meng et~al.(2019)Meng, Chen, Wang, Ma, and Liu]{meng2019convergence}
Q.~Meng, W.~Chen, Y.~Wang, Z.-M. Ma, and T.-Y. Liu.
\newblock Convergence analysis of distributed stochastic gradient descent with
  shuffling.
\newblock \emph{Neurocomputing}, 337:\penalty0 46--57, 2019.

\bibitem[Mishchenko et~al.(2020)Mishchenko, Khaled, and
  Richt{\'a}rik]{mishchenko2020random}
K.~Mishchenko, A.~Khaled, and P.~Richt{\'a}rik.
\newblock Random reshuffling: {S}imple analysis with vast improvements.
\newblock \emph{arXiv preprint arXiv:2006.05988}, 2020.

\bibitem[Nagaraj et~al.(2019)Nagaraj, Jain, and Netrapalli]{nagaraj2019sgd}
Dheeraj Nagaraj, Prateek Jain, and Praneeth Netrapalli.
\newblock Sgd without replacement: Sharper rates for general smooth convex
  functions.
\newblock In \emph{International Conference on Machine Learning}, pages
  4703--4711, 2019.

\bibitem[Nedi{\'c} and Bertsekas(2001)]{nedic2001convergence}
A.~Nedi{\'c} and D.~Bertsekas.
\newblock Convergence rate of incremental subgradient algorithms.
\newblock In \emph{Stochastic optimization: algorithms and applications}, pages
  223--264. Springer, 2001.

\bibitem[Nedic and Bertsekas(2001)]{nedic2001incremental}
A.~Nedic and D.~P. Bertsekas.
\newblock Incremental subgradient methods for nondifferentiable optimization.
\newblock \emph{SIAM J. on Optim.}, 12\penalty0 (1):\penalty0 109--138, 2001.

\bibitem[Nesterov(1983)]{Nesterov1983}
Y.~Nesterov.
\newblock A method for unconstrained convex minimization problem with the rate
  of convergence $\mathcal{O}(1/k^2)$.
\newblock \emph{Doklady AN SSSR}, 269:\penalty0 543--547, 1983.
\newblock Translated as Soviet Math. Dokl.

\bibitem[Nesterov(2004)]{Nesterov2004}
Y.~Nesterov.
\newblock \emph{{I}ntroductory lectures on convex optimization: {A} basic
  course}, volume~87 of \emph{Applied Optimization}.
\newblock Kluwer Academic Publishers, 2004.

\bibitem[Nguyen et~al.(2020)Nguyen, Tran-Dinh, Phan, Nguyen, and van
  Dijk]{nguyen2020unified}
L.~M. Nguyen, Q.~Tran-Dinh, D.~T. Phan, P.~H. Nguyen, and M.~van Dijk.
\newblock A unified convergence analysis for shuffling-type gradient methods.
\newblock \emph{arXiv preprint arXiv:2002.08246}, 2020.

\bibitem[Nguyen et~al.(2018)Nguyen, Nguyen, van Dijk, Richtarik, Scheinberg,
  and Takac]{Nguyen2018_sgdhogwild}
Lam Nguyen, Phuong~Ha Nguyen, Marten van Dijk, Peter Richtarik, Katya
  Scheinberg, and Martin Takac.
\newblock {SGD} and {H}ogwild! convergence without the bounded gradients
  assumption.
\newblock In \emph{Proceedings of the 35th International Conference on Machine
  Learning-Volume 80}, pages 3747--3755, 2018.

\bibitem[Paszke et al (2019)]{pytorch}
A.~Paszke {\emph{et al}}.
\newblock Pytorch: An imperative style, high-performance deep learning library.
\newblock In \emph{Advances in Neural Information Processing Systems 32}, pages
  8024--8035. Curran Associates, Inc., 2019.

\bibitem[Polyak(1964)]{polyak1964some}
B.~T. Polyak.
\newblock Some methods of speeding up the convergence of iteration methods.
\newblock \emph{USSR Computational Mathematics and Mathematical Physics},
  4\penalty0 (5):\penalty0 1--17, 1964.

\bibitem[Rajput et~al.(2020)Rajput, Gupta, and
  Papailiopoulos]{rajput2020closing}
S.~Rajput, A.~Gupta, and D.~Papailiopoulos.
\newblock Closing the convergence gap of {SGD} without replacement.
\newblock \emph{arXiv preprint arXiv:2002.10400}, 2020.

\bibitem[Robbins and Monro(1951)]{RM1951}
Herbert Robbins and Sutton Monro.
\newblock A stochastic approximation method.
\newblock \emph{The Annals of Mathematical Statistics}, 22\penalty0
  (3):\penalty0 400--407, 1951.

\bibitem[Ruder(2017)]{ruder2017overview}
Sebastian Ruder.
\newblock An overview of gradient descent optimization algorithms, 2017.

\bibitem[Safran and Shamir(2018)]{Safran2019HowGoodSGDShuffling}
I.~Safran and O.~Shamir.
\newblock How good is {SGD} with random shuffling?
\newblock \emph{arXiv preprint arXiv:1908.00045}, 2018.

\bibitem[Shamir(2016)]{shamir2016without}
O.~Shamir.
\newblock Without-replacement sampling for stochastic gradient methods.
\newblock In \emph{Advances in neural information processing systems}, pages
  46--54, 2016.

\bibitem[Smith(2017)]{smith2017cyclical}
L.~N. Smith.
\newblock Cyclical learning rates for training neural networks.
\newblock In \emph{2017 IEEE Winter Conference on Applications of Computer
  Vision (WACV)}, pages 464--472. IEEE, 2017.

\bibitem[Smith(2015)]{smith2015cyclical}
Leslie~N. Smith.
\newblock Cyclical learning rates for training neural networks, 2015.

\bibitem[Wang et~al.(2020)Wang, Nguyen, Bertozzi, Baraniuk, and
  Osher]{wang2020scheduled}
B.~Wang, T.~M. Nguyen, A.~L. Bertozzi, R.~G. Baraniuk, and S.~J. Osher.
\newblock Scheduled restart momentum for accelerated stochastic gradient
  descent.
\newblock \emph{arXiv preprint arXiv:2002.10583}, 2020.

\bibitem[Xiao et~al.(2017)Xiao, Rasul, and Vollgraf]{xiao2017fashion}
Han Xiao, Kashif Rasul, and Roland Vollgraf.
\newblock Fashion-mnist: a novel image dataset for benchmarking machine
  learning algorithms.
\newblock \emph{arXiv preprint arXiv:1708.07747}, 2017.

\bibitem[Ying et~al.(2017)Ying, Yuan, and Sayed]{ying2017convergence}
B.~Ying, K.~Yuan, and A.~H. Sayed.
\newblock Convergence of variance-reduced stochastic learning under random
  reshuffling.
\newblock \emph{arXiv preprint arXiv:1708.01383}, 2\penalty0 (3):\penalty0 6,
  2017.

\end{thebibliography}


==> sections/redundant.tex <==
\newpage
\section{Redundant Parts}

In this paper, we analyze convergence rates for the shuffling-type gradient method with mini-batch to solve~\eqref{ERM_problem_01} as described in Algorithm~\ref{sgd_shuffling_mb2}. 

\begin{algorithm}[hpt!]
   \caption{Shuffling-Type Gradient Method with Mini-Batch}
   \label{sgd_shuffling_mb2}
\begin{algorithmic}
   \STATE {\bfseries Initialization:} Choose an initial point $\tilde{w}_0\in\R^d$
   \STATE Mini-batch size $b \in [1,n]$ and number of mini-batches $m = n/b$
   \FOR{$t=1,2,\cdots,T $}
   \STATE Set $w_0^{(t)} := \tilde{w}_{t-1}$;
   \STATE Generate any permutation  $\sigma^{(t)}$ of $[n]$;
   \FOR{$i=0,\cdots, m -1$}
    \STATE Update $w_{i+1}^{(t)} := w_{i}^{(t)} - \eta_{i}^{(t)} \sum_{j=1}^b \nabla f ( w_i^{(t)} ; \sigma^{(t)} ( i b + j ) )$; 
   \ENDFOR
   \STATE Set $\tilde{w}_t := w_{m}^{(t)}$;
   \ENDFOR
   \STATE\textbf{Output:} Choose $\hat{w}_T$ which is a random iterate drawn from $\tilde{w}_{0},\cdots,\tilde{w}_{T-1}$ with probability 
\begin{align*}
    \mathbb{P}[\hat{w}_T = \tilde{w}_{t-1}] = \frac{\eta_t}{\sum_{t=1}^{T} \eta_t}, \ t = 1,\cdots,T. 
\end{align*}
\end{algorithmic}
\end{algorithm}

For the purpose of simplicity, we assume that the batch size divides the sample number evenly, that is, $n$ is divisible by $b$. Note that our analysis can be generalized for the case of arbitrary batch size using the same update rule and arguments. 

\section{Convergence Analysis - Regular Shuffling}\label{sec_analysis_shuffling}

% \begin{ass}\label{ass_bounded_variance}
% There exists non-negative constants $M, N \geq 0$ such that for any $w \in \R^d$ we have
% \begin{equation}\label{eq:bounded_variance}
%     \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) - \nabla F(w)}^2 \leq M \| \nabla F(w) \|^2 + N. 
% \end{equation}
% \end{ass}

In this paper, we analyze the case where the step size for every batch is the same within an epoch. Let us consider the learning rate given below: 
\begin{align*}
    \eta_i^{(t)} := \frac{\eta_t}{n}. 
\end{align*}
We have the following update for each epoch: 
\begin{align}\label{update_epoch}
    w_m^{(t)} = w_0^{(t)} - \frac{\eta_t}{n} \sum_{i=0}^{m-1} \sum_{j=1}^b \nabla f ( w_i^{(t)} ; \sigma^{(t)} ( i b + j ) ). 
\end{align}

We present our key lemma as follows. 
\begin{lem}\label{lem_basic_derivation_01}
Let $\sets{\tilde{w}_{t-1}}_{t = 1}^T$ be generated by Algorithm~\ref{sgd_shuffling_mb2} with $\eta_i^{(t)} = \frac{\eta_t}{n}$ such that $0 < \eta_t \leq \frac{1}{L}$.
Then, under Assumptions~\ref{ass_lower_bound}, \ref{ass_smooth}, and \ref{ass_bounded_gradient}, we have
\begin{align*}
    \mathbb{E}[\norms{ \nabla F( \hat{w}_T )  }^2] & =
        \frac{1}{\sum_{t=1}^{T} \eta_t} \sum_{t=1}^{T} \eta_t \norms{ \nabla F( \tilde{w}_{t-1} )  }^2 \\ & \leq \frac{2}{\sum_{t=1}^{T} \eta_t} [ F( \tilde{w}_{0} ) - F_* ] + \frac{L^2 G^2}{3} \frac{1}{\sum_{t=1}^{T} \eta_t} \sum_{t=1}^{T}  \eta_t^3 \tagthis \label{eq_lem_basic_derivation_01}, 
\end{align*}
where $\hat{w}_T$ is a random iterate drawn from $\tilde{w}_{0},\cdots,\tilde{w}_{T-1}$ with probability 
\begin{align*}
    \mathbb{P}[\hat{w}_T = \tilde{w}_{t-1}] = \frac{\eta_t}{\sum_{t=1}^{T} \eta_t}, \ t = 1,\dots,T,
\end{align*}
so that $\sum_{t=1}^{T} \mathbb{P}[\hat{w}_T = \tilde{w}_{t-1}] = 1$.
\end{lem}


\subsection{Exponential Learning Rate Schedule}
We consider the exponential learning rate schedule: 
\begin{align*}
    \eta_t = \eta \cdot \alpha^t, \ \text{for some } \alpha < 1, \ t \geq 1. \tagthis \label{exponential_learning_rate_01} 
\end{align*}

\begin{thm}\label{thm_exponential_LR}
Let $\sets{\tilde{w}_{t-1}}_{t = 1}^T$ be generated by Algorithm~\ref{sgd_shuffling_mb2} with $\eta_i^{(t)} = \frac{\eta_t}{n}$, where $\eta_t = \eta \cdot \alpha^t$ with $\alpha = \rho^{1/T} < 1$ and $\eta = \frac{\gamma}{T^{1/3}}$ for some $\gamma > 0$ such that $0 < \eta_t \leq \frac{1}{L}$.
Then, under Assumptions~\ref{ass_lower_bound}, \ref{ass_smooth}, and \ref{ass_bounded_gradient}, we have
\begin{align*}
    \mathbb{E}[\norms{ \nabla F( \hat{w}_T )  }^2] \leq \frac{1}{ T^{2/3}} \left( \frac{2 [ F( \tilde{w}_{0} ) - F_* ]}{\gamma \rho}  +   \frac{\gamma^2L^2 G^2}{3 \rho} \right) =  \Ocal\left( \frac{1}{T^{2/3}} \right), 
\end{align*}
where $\hat{w}_T$ is a random iterate drawn from $\tilde{w}_{0},\cdots,\tilde{w}_{T-1}$ with probability 
\begin{align*}
    \mathbb{P}[\hat{w}_T = \tilde{w}_{t-1}] = \frac{\eta_t}{\sum_{t=1}^{T} \eta_t}, \ t = 1,\dots,T,
\end{align*}
so that $\sum_{t=1}^{T} \mathbb{P}[\hat{w}_T = \tilde{w}_{t-1}] = 1$.
\end{thm}



\subsection{Cosine Learning Rate Schedule}

We consider the cosine learning rate schedule:
\begin{align*}
    \eta_t = \eta \left(1+ \cos \frac{t \pi}{T} \right), \ t \geq 1. \tagthis \label{cos_learning_rate_01} 
\end{align*}

\begin{thm}\label{thm_cos_LR}
Let $\sets{\tilde{w}_{t-1}}_{t = 1}^T$ be generated by Algorithm~\ref{sgd_shuffling_mb2} with $\eta_i^{(t)} = \frac{\eta_t}{n}$, where $\eta_t = \eta \left(1+ \cos \frac{t \pi}{T} \right)$ and $\eta = \frac{\gamma}{T^{1/3}}$ for some $\gamma > 0$ such that $0 < \eta_t \leq \frac{1}{L}$.
Then, under Assumptions~\ref{ass_lower_bound}, \ref{ass_smooth}, and \ref{ass_bounded_gradient}, and for $T\geq 2$, we have
\begin{align*}
    \mathbb{E}[\norms{ \nabla F( \hat{w}_T )  }^2] \leq \frac{1}{ T^{2/3}} \left( \frac{4 [ F( \tilde{w}_{0} ) - F_* ]}{\gamma }  +  \frac{8\gamma^2L^2 G^2}{3} \right) = \Ocal\left( \frac{1}{T^{2/3}} \right), 
\end{align*}
where $\hat{w}_T$ is a random iterate drawn from $\tilde{w}_{0},\cdots,\tilde{w}_{T-1}$ with probability 
\begin{align*}
    \mathbb{P}[\hat{w}_T = \tilde{w}_{t-1}] = \frac{\eta_t}{\sum_{t=1}^{T} \eta_t}, \ t = 1,\dots,T,
\end{align*}
so that $\sum_{t=1}^{T} \mathbb{P}[\hat{w}_T = \tilde{w}_{t-1}] = 1$.
\end{thm}


\begin{align}\label{sgd_momentum_shuffling}
    Shuffling
\end{align}
\section{Convergence Analysis - Momentum Shuffling}\label{sec_analysis_shuffling_momentum} 
\begin{thm}\label{thm_momentum}
Let $\{w_i^{(t)}\}$ be the sequence generated by Algorithm \ref{sgd_momentum_shuffling} with $\eta_i^{(t)} = \frac{\eta_t}{n}$ and $0 < \eta_t \leq \frac{1}{L}$ for every $t = 1, 2, \dots, T$.
Then, under Assumption \ref{ass_lower_bound}, \ref{ass_smooth}, and \ref{ass_bounded_gradient}, we have: 
\begin{align}
    \mathbb{E}\big[\| \nabla F( \hat{w}_T )  \|^2 \big] \leq    \frac{2 [F( \tilde{w}_{1} ) - F_*] + \eta_1 \norms{ \nabla F( \tilde{w}_{0} ) }^2 } {\big(\sum_{t=1}^T \eta_t \big)(1 - \beta^n)}   + \frac{4\beta^n G^2}{1 - \beta^n}    +   L^2 G^2  \frac{\sum_{t=1}^T \xi_t^3}{\sum_{t=1}^T \eta_t}.
    \tagthis \label{eq_thm_momentum}
\end{align}
where $\xi_t = \max (\eta_t, \eta_{t-1})$ for $t \geq 2$ and $\xi_1 = \eta_1$.
\end{thm}

\trang{Note: add the constant LR schedule.}

\subsection{Exponential Learning Rate Schedule}
We consider the exponential learning rate schedule: 
\begin{align*}
    \eta_t = \eta \cdot \alpha^t, \ \text{for some } \alpha < 1, \ t \geq 1. \tagthis \label{exponential_learning_rate} 
\end{align*}

\begin{thm}\label{thm_sgdm_exponential_LR}
Let $\sets{\tilde{w}_{t-1}}_{t = 1}^T$ be generated by Algorithm~\ref{sgd_momentum_shuffling} with $\eta_i^{(t)} = \frac{\eta_t}{n}$, where $\eta_t = \eta \cdot \alpha^t$ with $\alpha = \rho^{1/T} < 1$ and $\eta = \frac{\gamma}{T^{1/3}}$ for some $\gamma > 0$ such that $0 < \eta_t \leq \frac{1}{L}$. Let $\beta = (\frac{\delta}{T^{2/3}})^{1/n}$ for some $ \delta > 0$ such that $\beta < 1$.
Then, under Assumptions~\ref{ass_lower_bound}, \ref{ass_smooth}, and \ref{ass_bounded_gradient}, we have
\begin{align*}
    \mathbb{E}[\norms{ \nabla F( \hat{w}_T )  }^2] \leq  \Ocal\left( \frac{1}{T^{2/3}} \right), 
\end{align*}
where $\hat{w}_T$ is a random iterate drawn from $\tilde{w}_{0},\cdots,\tilde{w}_{T-1}$ with probability 
\begin{align*}
    \mathbb{P}[\hat{w}_T = \tilde{w}_{t-1}] = \frac{\eta_t}{\sum_{t=1}^{T} \eta_t}, \ t = 1,\dots,T,
\end{align*}
so that $\sum_{t=1}^{T} \mathbb{P}[\hat{w}_T = \tilde{w}_{t-1}] = 1$.
\end{thm}



\subsection{Cosine Learning Rate Schedule}

We consider the cosine learning rate schedule:
\begin{align*}
    \eta_t = \eta \left(1+ \cos \frac{t \pi}{T} \right), \ t \geq 1. \tagthis \label{cos_learning_rate} 
\end{align*}

\begin{thm}\label{thm_sgdm_cos_LR}
Let $\sets{\tilde{w}_{t-1}}_{t = 1}^T$ be generated by Algorithm~\ref{sgd_momentum_shuffling} with $\eta_i^{(t)} = \frac{\eta_t}{n}$, where $\eta_t = \eta \left(1+ \cos \frac{t \pi}{T} \right)$ and $\eta = \frac{\gamma}{T^{1/3}}$ for some $\gamma > 0$ such that $0 < \eta_t \leq \frac{1}{L}$. Let $\beta = (\frac{\delta}{T^{2/3}})^{1/n}$ for some $ \delta > 0$ such that $\beta < 1$.
Then, under Assumptions~\ref{ass_lower_bound}, \ref{ass_smooth}, and \ref{ass_bounded_gradient}, and for $T\geq 2$, we have
\begin{align*}
    \mathbb{E}[\norms{ \nabla F( \hat{w}_T )  }^2] \leq \Ocal\left( \frac{1}{T^{2/3}} \right), 
\end{align*}
where $\hat{w}_T$ is a random iterate drawn from $\tilde{w}_{0},\cdots,\tilde{w}_{T-1}$ with probability 
\begin{align*}
    \mathbb{P}[\hat{w}_T = \tilde{w}_{t-1}] = \frac{\eta_t}{\sum_{t=1}^{T} \eta_t}, \ t = 1,\dots,T,
\end{align*}
so that $\sum_{t=1}^{T} \mathbb{P}[\hat{w}_T = \tilde{w}_{t-1}] = 1$.
\end{thm}

\section{Proofs for SGD Shuffling with mini-batch}
\subsection*{Proof of Lemma~\ref{lem_basic_derivation_01}}

For each update $i \in [n]$, we have 
\begin{align*}
    w_i^{(t)} = w_0^{(t)} - \frac{\eta_t}{n} \sum_{k=0}^{i-1} \sum_{j=1}^b \nabla f ( w_k^{(t)} ; \sigma^{(t)} ( k b + j ) ). \tagthis \label{update_within}
\end{align*}
\textbf{For the bounded gradient assumption: }
Using this expression and the bounded gradient assumption \eqref{ass_bounded_gradient}, we can get: 
\begin{align*}
    \norms{ w_{i}^{(t)} - w_{0}^{(t)} }^2 &= \frac{\eta_t^2}{n^2} \Big\Vert \sum_{k=0}^{i-1} \sum_{j=1}^b \nabla f ( w_k^{(t)} ; \sigma^{(t)} ( k b + j ) ) \Big\Vert^2     \\
    & = \frac{i^2 b^2 \cdot \eta_t^2}{n^2} \Big\Vert \frac{1}{ib} \sum_{k=0}^{i-1} \sum_{j=1}^b \nabla f ( w_k^{(t)} ; \sigma^{(t)} ( k b + j ) )  \Big\Vert^2 \overset{\tiny\eqref{eq_bounded_gradient}}{\leq} \frac{i^2 b^2\cdot \eta_t^2}{n^2} G^2. 
    \tagthis \label{eq_bounded_01}
\end{align*}

\textbf{For the bounded variance assumption: }

Using this expression and the bounded variance assumption \eqref{ass_bounded_variance}, we can get:
\begin{align} 
    \norms{ w_{i}^{(t)} - w_{0}^{(t)} }^2 &= \frac{\eta_t^2}{n^2} \Big\Vert \sum_{k=0}^{i-1} \sum_{j=1}^b \nabla f ( w_k^{(t)} ; \sigma^{(t)} ( k b + j ) ) \Big\Vert^2     \\
    %
    & = \frac{i^2 b^2 \cdot \eta_t^2}{n^2} \Big\Vert \frac{1}{ib} \sum_{k=0}^{i-1} \sum_{j=1}^b \nabla f ( w_k^{(t)} ; \sigma^{(t)} ( k b + j ) )  \Big\Vert^2  \\
    %
    & \leq \frac{3 i^2 \eta_t^2}{m^2}  \Big\Vert \frac{1}{ib} \sum_{k=0}^{i-1} \sum_{j=1}^b \left(\nabla f ( w_k^{(t)} ; \sigma^{(t)} ( k b + j ) ) - \nabla f ( w_0^{(t)} ; \sigma^{(t)} ( k b + j ) ) \right) \Big\Vert^2   \\
    &+ \frac{3 i^2 \eta_t^2}{m^2} \Big(\Big\Vert \frac{1}{ib} \sum_{k=0}^{i-1} \sum_{j=1}^b \left(\nabla f ( w_0^{(t)} ; \sigma^{(t)} ( k b + j ) ) - \nabla F ( w_0^{(t)}) \right) \Big\Vert^2 +  \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 \Big)   \\
    %
    & \leq \frac{3 i^2 \eta_t^2}{m^2}  \frac{1}{ib} \sum_{k=0}^{i-1} \sum_{j=1}^b \Big\Vert \nabla f ( w_k^{(t)} ; \sigma^{(t)} ( k b + j ) ) - \nabla f ( w_0^{(t)} ; \sigma^{(t)} ( k b + j ) )  \Big\Vert^2   \\
    &+ \frac{3 i^2 \eta_t^2}{m^2} \Big( \frac{1}{ib} \sum_{k=0}^{i-1} \sum_{j=1}^b \Big\Vert  \nabla f ( w_0^{(t)} ; \sigma^{(t)} ( k b + j ) ) - \nabla F ( w_0^{(t)})  \Big\Vert^2 +  \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 \Big)  \\
    %
    & \leq \frac{3 i^2 \eta_t^2}{m^2}  \frac{L^2}{ib}  \sum_{k=0}^{i-1} \sum_{j=1}^b \Big\Vert w_k^{(t)} - w_0^{(t)}   \Big\Vert^2   \\
    &+ \frac{3 i^2 \eta_t^2}{m^2} \Big( \frac{1}{ib} \sum_{j=1}^n \Big\Vert  \nabla f ( w_0^{(t)} ; j ) - \nabla F ( w_0^{(t)})  \Big\Vert^2 +  \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 \Big)   \\
    %
    & \leq \frac{3 i^2 \eta_t^2}{m^2}  \frac{L^2}{i} I 
    + \frac{3 i^2 \eta_t^2}{m^2} \left( \frac{1}{ib} n \Big(M  \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 + N\Big) +  \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 \right) 
     \\
    %
    & \leq \frac{3 i L^2 \eta_t^2}{m^2} I 
    + \frac{3 \eta_t^2}{m^2} \left( \frac{in}{b} \Big(M  \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 + N\Big) + i^2 \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 \right) \tagthis \label{eq_bounded_var}
\end{align}
 where 
\begin{align*}
    I = \sum_{i=0}^{m-1} \Big\Vert w_i^{(t)} - w_0^{(t)}   \Big\Vert^2
\end{align*}
 
\begin{align*}
    I &= \sum_{i=0}^{m-1} \Big\Vert w_i^{(t)} - w_0^{(t)}   \Big\Vert^2\\
    & \leq \frac{3 L^2 \eta_t^2}{m^2} I \sum_{i=0}^{m-1} i
    + \frac{3 \eta_t^2}{m^2} \left( \sum_{i=0}^{m-1} i \frac{n}{b} \Big(M  \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 + N\Big) + \sum_{i=0}^{m-1} i^2 \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 \right)\\
    %
    & \leq \frac{3 L^2 \eta_t^2}{2} I 
    + \frac{3 \eta_t^2}{m^2} \left( \frac{m^3}{2}  \Big(M  \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 + N\Big) + \frac{m^3}{3} \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 \right) \\
    %
    & \leq \frac{3}{4} I 
    + \frac{ m \eta_t^2}{2} \left( (3M + 2) \Big\Vert  \nabla F ( w_0^{(t)})\Big\Vert^2 + N \right)
\end{align*}



From the assumption \eqref{ass_smooth} that $F$ is $L$-smooth and the update rule for an epoch, we obtain that: 
\begin{align*} 
    F( w_0^{(t+1)} )  & \overset{\eqref{eq:Lsmooth}}{\leq} F( w_0^{(t)} ) + \nabla F( w_0^{(t)} )^{\top}(w_0^{(t+1)} - w_0^{(t)}) + \frac{L}{2}\norms{w_0^{(t+1)} - w_0^{(t)}}^2  \\
    &\overset{\eqref{update_epoch}}{=} F( w_0^{(t)} ) - \eta_t \nabla F( w_0^{(t)} )^{\top} \left( \frac{1}{n}\sum_{i=0}^{m-1} \sum_{j=1}^b \nabla f ( w_i^{(t)} ; \sigma^{(t)} ( i b + j ) )\right)  \\
    & \quad + \frac{L \eta_t^2}{2} \Big \Vert \frac{1}{n} \sum_{i=0}^{m-1} \sum_{j=1}^b \nabla f ( w_i^{(t)} ; \sigma^{(t)} ( i b + j ) \Big\Vert ^2  \\
    %
    & \overset{\tiny(a)}{=} F( w_0^{(t)} ) - \frac{\eta_t}{2} \norms{ \nabla F( w_0^{(t)} )}^2 + \frac{\eta_t}{2} \Big\Vert \nabla F( w_0^{(t)} )  - \frac{1}{n}\sum_{i=0}^{m-1} \sum_{j=1}^b \nabla f ( w_i^{(t)} ; \sigma^{(t)} ( i b + j ) )\Big\Vert^2  \\
    & \quad - \frac{\eta_t}{2} \left( 1 - L\eta_t  \right) \Big\Vert \frac{1}{n}\sum_{i=0}^{m-1} \sum_{j=1}^b \nabla f ( w_i^{(t)} ; \sigma^{(t)} ( i b + j )\Big\Vert^2   \\
    & \leq F( w_0^{(t)} ) - \frac{\eta_t}{2} \norms{ \nabla F( w_0^{(t)} )}^2 + \frac{\eta_t}{2} \Big\Vert \nabla F( w_0^{(t)} )  - \frac{1}{n}\sum_{i=0}^{m-1} \sum_{j=1}^b \nabla f ( w_i^{(t)} ; \sigma^{(t)} ( i b + j ) )\Big\Vert^2, \tagthis \label{eq_bounded_02}
\end{align*}
where (\textit{a}) follows from the equality $u^{\top}v = \frac{1}{2}(\norms{u}^2 + \norms{v}^2 - \norms{u - v}^2)$ and the last equality comes from the fact that $\eta_t \leq \frac{1}{L}$.

%Because of the fact that $\eta_t \leq \frac{1}{L}$, we obtain that

Now we use an interesting fact from the permutation $\sigma^{(t)}$ to rewrite the full gradient $\nabla F( w_0^{(t)} )$ and bound the following term:
\begin{align*} 
    &  \frac{\eta_t}{2} \Big\Vert \nabla F( w_0^{(t)} )  - \frac{1}{n}\sum_{i=0}^{m-1} \sum_{j=1}^b \nabla f ( w_i^{(t)} ; \sigma^{(t)} ( i b + j ) )\Big\Vert^2  \\
    %
    & = \frac{\eta_t}{2} \Big\Vert \frac{1}{n}\sum_{i=0}^{m-1} \sum_{j=1}^b \Big(\nabla f ( w_0^{(t)} ; \sigma^{(t)} ( i b + j ) )  -  \nabla f ( w_i^{(t)} ; \sigma^{(t)} ( i b + j ) ) \Big) \Big\Vert^2  \\
    %
    & \overset{\tiny(b)}{\leq} \frac{\eta_t}{2n} \sum_{i=0}^{m-1} \sum_{j=1}^b \Big\Vert \nabla f ( w_0^{(t)} ; \sigma^{(t)} ( i b + j ) )  -  \nabla f ( w_i^{(t)} ; \sigma^{(t)} ( i b + j ) )  \Big\Vert^2  \\
    %
    & \leq \frac{L^2\eta_t}{2n} \sum_{i=0}^{m-1} \sum_{j=1}^b \Big\Vert w_0^{(t)} - w_i^{(t)}  \Big\Vert^2  
    %
    \ \ \overset{\eqref{eq_bounded_01}}{\leq} \frac{L^2 \eta_t}{2n}  \sum_{i=0}^{m-1} \sum_{j=1}^b \frac{i^2 b^2 \cdot \eta_t^2}{n^2} G^2 
    %
    \ \ \overset{\tiny(c)}{\leq}\frac{L^2 G^2}{6} \cdot  \eta_t^3, \tagthis \label{eq_bounded_03}
\end{align*}
where (\textit{b}) is from the Cauchy-Schwarz inequality, and (\textit{c}) follows from the facts that $\sum_{i=0}^{m-1} i^2  \leq \frac{m^3}{3}$ and $n = mb$. We also use the previous expression \eqref{eq_bounded_01} to bound the distance between the updates.  

Using \eqref{eq_bounded_03} in the derived inequality \eqref{eq_bounded_02} with a note that $\tilde{w}_t = w_0^{(t+1)}$ and $\tilde{w}_{t-1} = w_0^{(t)}$, we obtain:
\begin{align*}
    F( \tilde{w}_{t} ) \leq F(\tilde{w}_{t-1} ) - \frac{\eta_t}{2} \norms{ \nabla F( \tilde{w}_{t-1} )  }^2 + \frac{L^2 G^2}{6} \cdot  \eta_t^3,
\end{align*}
which is equivalent to
\begin{align*}
    \eta_t \norms{ \nabla F( \tilde{w}_{t-1} )  }^2  
    \leq 2 \big( F(\tilde{w}_{t-1} ) - F( \tilde{w}_{t} ) \big) + \frac{L^2 G^2}{3} \cdot  \eta_t^3.
\end{align*}
Summing the last inequality for $t =  1, \dots, T$, we get: 
\begin{align*}
    & \sum_{t=1}^{T}\eta_t \norms{ \nabla F( \tilde{w}_{t-1} )  }^2  
    \leq 2 \big( F(\tilde{w}_{0} ) - F_* \big) + \frac{L^2 G^2}{3}  \sum_{t=1}^{T} \eta_t^3.
\end{align*}
Hence, dividing by $\sum_{t=1}^T \eta_t$ to both sides, the desired result follows immediately.

\subsection*{Proof of Theorem~\ref{thm_exponential_LR}}

From the exponential learning rate scheme and $\alpha < 1$ we have
\begin{align}
    \sum_{t=1}^{T} \eta_t = \eta \sum_{t=1}^{T} \alpha^t \geq \eta \sum_{t=1}^{T} \alpha^T = \eta T \cdot\alpha^T = \eta \rho T, \tagthis \label{eq_exp_eta_t}
\end{align}
and 
\begin{align}
    \sum_{t=1}^{T} \eta_t^3 = \eta^3 \sum_{t=1}^{T} \alpha^{3t} \leq \eta^3 \sum_{t=1}^{T} 1  = \eta^3   T. \tagthis \label{eq_exp_eta_t^3}
\end{align}

Using these facts in Lemma~\ref{lem_basic_derivation_01}, we have the following:
\begin{align*}
    \mathbb{E}[\norms{ \nabla F( \hat{w}_T )  }^2]  & \ \ \leq \frac{2}{\sum_{t=1}^{T} \eta_t} [ F( \tilde{w}_{0} ) - F_* ] + \frac{L^2 G^2}{3} \frac{1}{\sum_{t=1}^{T} \eta_t} \sum_{t=1}^{T}  \eta_t^3 \\ 
    & \overset{\eqref{eq_exp_eta_t}\eqref{eq_exp_eta_t^3}}{\leq} \frac{2}{\eta \rho T} [ F( \tilde{w}_{0} ) - F_* ] + \frac{L^2 G^2}{3} \cdot \frac{\eta^2}{\rho }   \\
    & \ \ = \frac{2}{\gamma \rho T^{2/3}} [ F( \tilde{w}_{0} ) - F_* ] +  \frac{1}{ T^{2/3}} \frac{\gamma^2L^2 G^2}{3 \rho}, 
\end{align*}
where the last equality comes from the fact that $\eta = \frac{\gamma}{T^{1/3}}$ for some $\gamma > 0$. 
This is the estimated convergence rate for Algorithm~\ref{sgd_shuffling_mb2}:
\begin{align*}
    \mathbb{E}[\norms{ \nabla F( \hat{w}_T )  }^2]   \leq \frac{1}{ T^{2/3}} \left( \frac{2 [ F( \tilde{w}_{0} ) - F_* ]}{\gamma \rho}  +   \frac{\gamma^2L^2 G^2}{3 \rho} \right) = \Ocal\left( \frac{1}{T^{2/3}} \right).
\end{align*}
This completes the proof. 

\subsection*{Proof of Theorem~\ref{thm_cos_LR}}
First, let us prove an elementary result regarding to the sum: $A = \sum_{t=1}^T \cos \frac{t \pi}{T}$.

Multiplying this sum with the term $\sin \frac{\pi}{2T}$, we get: 
\begin{align*}
    A \cdot \sin \frac{\pi}{2T} &= \sum_{t=1}^T \cos \frac{t \pi}{T} \sin \frac{\pi}{2T} 
    \overset{(a)}{=} \frac{1}{2} \sum_{t=1}^T \Big( \sin \frac{(2t+1) \pi}{2T} - \sin \frac{ (2t-1) \pi}{2T} \Big) \\
    &=  \frac{1}{2} \Big( \sin \frac{(2T+1) \pi}{2T} - \sin \frac{ \pi}{2T} \Big) 
    = \frac{1}{2} \Big( - \sin \frac{\pi}{2T} - \sin \frac{\pi}{2T} \Big) = - \sin \frac{\pi}{2T}.
\end{align*}
where (\textit{a}) comes from the identity
$\cos a \cdot \sin b = \frac{1}{2} (\sin (a+b) - \sin (a-b))$.

Because $\sin \frac{\pi}{2T}$ is nonzero, we get the result $A = \sum_{t=1}^T \cos \frac{t \pi}{T}  = -1.$ 

Now we are ready to take the sum of cosine learning rates:
\begin{align*}
    \sum_{t=1}^{T} \eta_t = \eta \sum_{t=1}^{T} \left(1+ \cos \frac{t \pi}{T} \right)  = \eta (T-1) \geq \frac{\eta T}{2}, \ \text{for} \ T \geq 2. \tagthis \label{eq_cos_eta_t}
\end{align*}
Also from the fact that $1+ \cos \frac{T \pi}{T} = 0$ and $1+ \cos \frac{t \pi}{T}  \leq 2$, we can bound:
\begin{align*}
    \sum_{t=1}^{T} \eta_t^3 = \eta^3 \sum_{t=1}^{T} \left(1+ \cos \frac{t \pi}{T} \right)^3 = \eta^3 \sum_{t=1}^{T-1} \left(1+ \cos \frac{t \pi}{T} \right)^3 \leq  \eta^3 \sum_{t=1}^{T-1} 2^3  = 8 \eta^3 (T-1). \tagthis \label{eq_cos_eta_t^3}
\end{align*}

Applying these inequalities in Lemma~\ref{lem_basic_derivation_01}, we obtain that:
\begin{align*}
    \mathbb{E}[\norms{ \nabla F( \hat{w}_T )  }^2]  & \ \ \leq \frac{2}{\sum_{t=1}^{T} \eta_t} [ F( \tilde{w}_{0} ) - F_* ] + \frac{L^2 G^2}{3} \frac{1}{\sum_{t=1}^{T} \eta_t} \sum_{t=1}^{T}  \eta_t^3 \\ 
    & \overset{\eqref{eq_cos_eta_t}\eqref{eq_cos_eta_t^3}}{\leq} \frac{4}{\eta T} [ F( \tilde{w}_{0} ) - F_* ] + \frac{L^2 G^2}{3} \cdot 8\eta^2   \\
    & \ \ = \frac{4}{\gamma T^{2/3}} [ F( \tilde{w}_{0} ) - F_* ] +  \frac{8\gamma^2}{ T^{2/3}} \frac{L^2 G^2}{3}, 
\end{align*}
where the last equality follows from the fact that $\eta = \frac{\gamma}{T^{1/3}}$ for some $\gamma > 0$. 

Hence we get the desired convergence rate for cosine learning rate scheme:
\begin{align*}
    \mathbb{E}[\norms{ \nabla F( \hat{w}_T )  }^2]   \leq \frac{1}{ T^{2/3}} \left( \frac{4 [ F( \tilde{w}_{0} ) - F_* ]}{\gamma }  +  \frac{8\gamma^2L^2 G^2}{3} \right) = \Ocal\left( \frac{1}{T^{2/3}} \right).
\end{align*}
This completes the proof.



% ==========================================

% \newpage
% \section*{Redundant}

% Let 
% \begin{align*}
%     \alpha = 1 - \frac{1}{T^{\beta}} < 1, \ \text{for some } \beta \geq 1 \tagthis \label{alpha_choice}
% \end{align*}

% We have
% \begin{align*}
%     \mathbb{E}[\norms{ \nabla F( \hat{w}_T )  }^2] & \leq \frac{\frac{1}{T^{\beta}}}{\left( 1 - \left( 1 - \frac{1}{T^{\beta}} \right)^T \right)} \cdot \frac{2}{\eta \left( 1 - \frac{1}{T^{\beta}} \right) } [ F( \tilde{w}_{0} ) - F_* ] + \eta^2 L^2 G^2. \tagthis \label{eq_002}
% \end{align*}

% Note that if $T$ is large enough
% \begin{align*}
%     \frac{\frac{1}{T^{\beta}}}{\left( 1 - \left( 1 - \frac{1}{T^{\beta}} \right)^T \right)} \approx \frac{\frac{1}{T^{\beta}}}{\left( 1 - \left( 1 - \frac{1}{T^{\beta-1}} \right) \right)} = \frac{1}{T}. 
% \end{align*}

% Therefore, with the choice of $\eta = \frac{\gamma}{T^{1/3}}$ for some $\gamma > 0$, we have
% \begin{align*}
%     \mathbb{E}[\norms{ \nabla F( \hat{w}_T )  }^2] \leq \frac{2}{ T^{2/3} \left( 1 - \frac{1}{T^{\beta}} \right) \gamma } [ F( \tilde{w}_{0} ) - F_* ] + \frac{\gamma^2 L^2 G^2}{T^{2/3}} =  \Ocal\left( \frac{1}{T^{2/3}} \right). 
% \end{align*}

% The learning rate choice becomes
% \begin{align*}
%     \eta_t = \frac{\gamma}{T^{1/3}} \left( 1 - \frac{1}{T^{\beta}} \right)^t, \ \text{for some } \gamma > 0 \text{ and some } \beta \geq 1. 
% \end{align*}

% \textbf{ANOTHER CHOICE}. Note that we can choose 
% \begin{align*}
%     \alpha = \left( \frac{\delta}{T}  \right)^{1/T} < 1, \ \text{for some } \delta > 0. 
% \end{align*}

% Note that
% \begin{align*}
%     \frac{(1 - \alpha)}{(1 - \alpha^T)} = \frac{\left(1 - \left( \frac{\delta}{T}  \right)^{1/T} \right)}{(1 - \frac{\delta}{T})} & = \frac{\left( 1 - \exp\left( \frac{1}{T} \ln\left( \frac{\delta}{T} \right) \right) \right)}{(1 - \frac{\delta}{T})} \approx \frac{\left( 1 - \exp\left( - \frac{1}{T} \right) \right)}{(1 - \frac{\delta}{T})} \approx \frac{\frac{1}{T}}{(1 - \frac{\delta}{T})}
%      \approx \frac{1}{T}. 
% \end{align*}
% The learning rate choice becomes
% \begin{align*}
%     \eta_t = \frac{\gamma}{T^{1/3}} \left( \left( \frac{\delta}{T}  \right)^{1/T} \right)^t, \ \text{for some } \gamma > 0 \text{ and some } \delta > 0. 
% \end{align*}

% We have 
% \begin{align*}
%     \frac{1}{I} = \sum_{t=1}^T \alpha^t = \frac{\alpha(1 - \alpha^T)}{1 - \alpha}  \leq T\\
% \end{align*}
% Therefore $I \geq 1/T.$
% \begin{align*}
%     &I = \frac{(1 - \alpha)}{ \alpha (1 - \alpha^T)} = \left( \frac{1}{\alpha} - 1 \right) \frac{1}{1 - \alpha^T}\\
%     &I = \left( \Big(\frac{T}{\delta}\Big)^{1/T} - 1 \right) \frac{1}{(1 - \frac{\delta}{T})} 
%     \overset{(a)}{=} \left( \ln \Big(\frac{T}{\delta}\Big) \frac{1}{T} + o \Big(\frac{1}{T}\Big)\right) \frac{T}{(T - \delta)} \text{ for } \alpha = \left( \frac{\delta}{T}  \right)^{1/T} < 1.\\
% \end{align*}
% where (a) comes from the definition of derivative: 
% $f(x + \epsilon) - f(x) = f'(x) \cdot \epsilon + o(\epsilon)$.

% Apply this for $f(x) = a^x$, $f'(x) = a^x \ln (a)$ at $a = T/\delta$, $x = 0$ and $\epsilon = 1/T$ we get

% $ \Big(\frac{T}{\delta}\Big)^{1/T} - 1 = ln\Big(\frac{T}{\delta}\Big) \frac{1}{T} + o \Big(\frac{1}{T}\Big)$

% Note: choosing $\alpha = \delta^{1/T} < 1$ will be much more simple: 
% \begin{align*}
%     \sum_{t=1}^T \eta_t \geq T \eta_T = T \delta.
% \end{align*}

% \lam{Note: Show that
% \begin{itemize}
%     \item There exists $\hat{T} > 0$ such that $\forall T \geq \hat{T}$: $\left( \frac{T}{\delta}  \right)^{\frac{1}{T}} - 1 \leq \frac{\ln\left(\frac{T}{\delta}\right) + 1 }{T}$
%     \item There exists $\hat{T} > 0$ such that $\forall T \geq \hat{T}$: $\left( 1 - \frac{1}{T^{\beta - 1} \ln(T)}  \right) \geq \left( 1 - \frac{1}{T^{\beta}} \right)^T$
% \end{itemize}
% }


% \textbf{QUESTION}: 
% \begin{itemize}
%     \item What are the best values of $\alpha < 1$ and $\eta > 0$ so that $\frac{(1 - \alpha)}{\eta \cdot \alpha (1 - \alpha^T)}$ and $\eta^2$ could be minimized (w.r.t. $T$)? 
%     \item Can we find $\alpha < 1$ (depending on $T$) such that $\frac{(1 - \alpha)}{\alpha (1 - \alpha^T)} \approx \frac{1}{T^{\beta}}$ for some $\beta > 1$? 
    
%     \trang{No? Because $\frac{(1 - \alpha)}{\alpha (1 - \alpha^T)}$ is actually $\frac{1}{\sum_{t=1}^T \alpha^t}$. 
%     We require $\sum_{t=1}^T \alpha^t$ to grow with a rate $T^\beta$ for $\beta > 1$, which is larger than $T$, while $\sum_{t=1}^T \alpha^t < T$ because $\alpha < 1$. }
% \end{itemize}


\section{SGD Shuffling with Momentum}



% \begin{ass}\label{ass_bounded_gradient}
% There exists a constant $G > 0$ such that $\forall w \in \mathbb{R}^d$, we have
% \begin{equation}\label{eq_bounded_gradient}
%     \norms{ \nabla f(w; i ) }^2 \leq G^2,~~~\forall i \in [n].
% \end{equation}
% \end{ass} 

\textbf{Notation.} 

Recall that $g_{i}^{(t)} = \nabla f ( w_{i}^{(t)} ; \sigma^{(t)} ( i + 1 ) ) $ is the $(i+1)$-th gradient at epoch $t$. 

We also denote the following terms: 
\begin{align*}
    h_{i}^{(t)} &= g_{i}^{(t)} - \nabla f ( w_{0}^{(t)} ; \sigma^{(t)} ( i + 1 ) ) \\
    k_{i}^{(t-1)} &= g_{i}^{(t-1)} - \nabla f ( w_{0}^{(t)} ; \sigma^{(t)} ( i + 1 ) ) 
\end{align*}


\begin{lem}\label{lem_bounded_momentum}
For all $t = 1, 2, \dots, T$ and $i=0,\cdots,n-1$, we have
\begin{equation}\label{eq_bounded_momentum}
    \norms{ m_{i+1}^{(t)} }^2 \leq G^2.
\end{equation}
\end{lem}
From this lemma we have a side note that 
\begin{align*}
    \Big\Vert\frac{1}{n} \sum_{i=0}^{n-1} m_{i+1}^{(t)} \Big\Vert^2 \leq G^2.
\end{align*}
and also
\begin{align*}
    \Big\Vert\nabla F( w_0^{(t)} ) \Big\Vert^2 = \Big\Vert \frac{1}{n} \sum_{i=0}^{n-1} \nabla f ( w_{0}^{(t)} ; \sigma^{(t)} ( i + 1 ) ) \Big\Vert^2 \leq G^2.
\end{align*}
for every $t = 1, 2, \dots, T$.
\begin{proof} 
We proof Lemma~\ref{lem_bounded_momentum} by induction. First, we can see that $\norms{ m_{0}^{(1)} }^2 = \norms{ \tilde{m}_{0}}^2 = 0 \leq G^2$. 
Assume that for the first epoch $t = 1$, the statement is true for $i = k-1$ , that is:  
\begin{equation*}
    \norms{ m_{k}^{(1)} }^2 \leq G^2.
\end{equation*}
By the update rule $m_{k+1}^{(1)} = \beta m_{k}^{(1)} + (1-\beta) g_{k}^{(1)}$ and the convexity of squared norm function, we obtain that: 
\begin{equation*}
    \Big\Vert m_{k+1}^{(1)} \Big\Vert^2  \leq  \beta \Big\Vert m_{k}^{(1)} \Big\Vert^2 + (1-\beta) \Big\Vert g_{k}^{(1)} \Big\Vert^2  \leq  \beta G^2 + (1-\beta) G^2 = G^2, 
\end{equation*}
where the induction hypothesis and assumption~\ref{ass_bounded_gradient} apply in the last inequality. 

Since the statement \eqref{eq_bounded_momentum} holds for $i = k, t= 1$; it is true for all iterations $i = 0, \dots, n - 1$ of the first epoch. 

Using the same argument, we obtain that the statement is satisfied for every epoch $t = 1, 2, \dots, T$ and all iterations $i = 0, \dots, n - 1$. 

\end{proof}

\begin{lem} \label{lem_bounded_02}
For $i = 0, 1, ... ,n-1$ and $t\geq 2$; we have this bound
\begin{align*}
    \max \Big( \Big \Vert h_{i}^{(t)} \Big \Vert^2; \Big \Vert k_{i}^{(t-1)} \Big \Vert^2 \Big) \leq L^2 G^2 \xi_t^2
\end{align*}
where $\xi_t = \max (\eta_t; \eta_{t-1}).$ 
\end{lem}
%(\lam{Maybe better to write $\xi_t^2 = \max (\eta_t^2; \eta_{t-1}^2)$}).
%\trang{We changed it back because we will need to use that later.}

\begin{proof}
At first using the $L$-smooth assumption we obtain that: 
\begin{align*}
    \Big \Vert h_{i}^{(t)} \Big \Vert^2 &= \Big \Vert\nabla f ( w_{i}^{(t)} ; \sigma^{(t)} ( i + 1 ) ) - \nabla f ( w_{0}^{(t)} ; \sigma^{(t)} ( i + 1 ) ) \Big \Vert^2 \leq L^2 \Big \Vert w_{i}^{(t)} - w_{0}^{(t)} \Big \Vert^2    \\
    %
    \Big \Vert k_{i}^{(t-1)} \Big \Vert^2 &= \Big \Vert \nabla f ( w_{i}^{(t-1)} ; \sigma^{(t-1)} ( i + 1 ) ) - \nabla f ( w_{0}^{(t)} ; \sigma^{(t)} ( i + 1 ) ) \Big \Vert^2 \leq L^2 \Big \Vert w_{i}^{(t-1)} - w_{0}^{(t)} \Big \Vert^2
\end{align*}
\trang{This is where we need the same permutation.}

Now from the update $w_{i+1}^{(t)} := w_{i}^{(t)} - \eta_i^{(t)} m_{i+1}^{(t)}$ in Algorithm~\ref{sgd_momentum_shuffling} with $\eta_i^{(t)} := \frac{\eta_t}{n}$, for $i =  1, ... ,n-1$, we have:
\begin{align*}
    w_{i}^{(t)} &= w_{i-1}^{(t)} - \frac{\eta_t}{n} m_{i}^{(t)} = w_{0}^{(t)} - \frac{\eta_t}{n} \sum_{j=0}^{i-1} m_{j+1}^{(t)} ;  \tagthis \label{update_momentum_epoch}\\
    w_{0}^{(t)} = w_{n}^{(t-1)} &= w_{n-1}^{(t-1)} - \frac{\eta_{t-1}}{n} m_{n}^{(t-1)} = w_{i}^{(t-1)} - \frac{\eta_{t-1}}{n} \sum_{j = i}^{n-1} m_{j+1}^{(t-1)} .  
\end{align*}

Hence, for $i =  0, 1, ... ,n-1$, using these expressions and the bounded momentum lemma \eqref{eq_bounded_momentum}, we can bound
\begin{align*}
    \norms{ w_{i}^{(t)} - w_{0}^{(t)} }^2 &= \eta_t^2 \Big\Vert \frac{1}{n} \sum_{j=0}^{i-1} m_{j+1}^{(t)}  \Big\Vert^2  
     \overset{\tiny\eqref{eq_bounded_momentum}}{\leq}  \eta_t^2 G^2.   \\
    %
    \norms{ w_{i}^{(t-1)} - w_{0}^{(t)} }^2 &= \eta_{t-1}^2 \Big\Vert \frac{1}{n} \sum_{j = i}^{n-1} m_{j+1}^{(t-1)} \Big\Vert^2  
     \overset{\tiny\eqref{eq_bounded_momentum}}{\leq}  \eta_{t-1}^2 G^2.   
\end{align*}
Now we are ready to have the desired result for $i =  0, 1, ... ,n-1$: 
\begin{align*}
    \max \Big( \Big \Vert h_{i}^{(t)} \Big \Vert^2; \Big \Vert k_{i}^{(t-1)} \Big \Vert^2 \Big) &\leq L^2 \max \Big( \eta_t^2 G^2; \eta_{t-1}^2 G^2\Big)  \\ %(\lam{\leq})
    &\leq  L^2 G^2 \max \big(\eta_t^2; \eta_{t-1}^2\big) = L^2 G^2 \max (\eta_t; \eta_{t-1})^2 = L^2 G^2 \xi_t^2;
\end{align*}
where the last line follows since $\eta_t > 0$ and $\eta_{t-1}>0$.
\end{proof}

We have the following lemma that rewrite the momentum: 
\begin{lem} \label{lem_momentum_formula}
For $i = 0, 1, \dots, n-1$ and $t\geq 2$ we have 
\begin{align*}
    m_{i+1}^{(t)} 
    &= \beta^{n} m_{i+1}^{(t-1)} + (1-\beta) \Big(\beta^{n-1} g_{i+1}^{(t-1)} + \dots + \beta^{i+1} g_{n-1}^{(t-1)} + \beta^i g_{0}^{(t)} + \dots +  \beta g_{i-1}^{(t)} + g_{i}^{(t)} \Big).
\end{align*}
From this expression we obtain the following sum: 
\begin{align*} 
    \frac{1}{n} \sum_{i=0}^{n-1} m_{i+1}^{(t)} = \beta^n I +  J \tagthis \label{eq_formula_sum}
\end{align*}
where
\begin{align*}
    I = \frac{1}{n} \sum_{i=0}^{n-1} m_{i+1}^{(t-1)} \ \text{and} \ 
    J = \frac{1-\beta}{n} \sum_{i=0}^{n-1} \left[  \left( \sum_{j=n-i}^{n-1} \beta^{j} \right) g_{i}^{(t-1)} +  \left( \sum_{j=0}^{n-i-1} \beta^{j} \right) g_{i}^{(t)}  \right]
\end{align*}
\end{lem}

\begin{proof}
The first statement follows directly from the momentum update rule: 
\begin{align*}
    m_{i+1}^{(t)} &= \beta m_{i}^{(t)} + (1-\beta) g_{i}^{(t)} %\\
    %&= \beta \Big( \beta m_{i-1}^{(t)} + (1-\beta) g_{i-1}^{(t)}  \Big) + (1-\beta) g_{i}^{(t)} \\
    = \beta^2 m_{i-1}^{(t)} + (1-\beta) \beta g_{i-1}^{(t)} + (1-\beta) g_{i}^{(t)} \\ 
    &= \beta^{i+1} m_{0}^{(t)} + (1-\beta) \Big( \beta^i g_{0}^{(t)} + \dots +  \beta g_{i-1}^{(t)} + g_{i}^{(t)} \Big) \\ 
    &\overset{(a)}{=} \beta^{i+1} m_{n}^{(t-1)} + (1-\beta) \Big( \beta^i g_{0}^{(t)} + \dots +  \beta g_{i-1}^{(t)} + g_{i}^{(t)} \Big) \\
    %&= \beta^{i+2} m_{n-1}^{(t-1)} + (1-\beta) \Big(\beta^{i+1} g_{n-1}^{(t-1)} + \beta^i g_{0}^{(t)} + \dots +  \beta g_{i-1}^{(t)} + g_{i}^{(t)} \Big) \\
    &= \beta^{n} m_{i+1}^{(t-1)} + (1-\beta) \Big(\beta^{n-1} g_{i+1}^{(t-1)} + \dots + \beta^{i+1} g_{n-1}^{(t-1)} + \beta^i g_{0}^{(t)} + \dots +  \beta g_{i-1}^{(t)} + g_{i}^{(t)} \Big) 
\end{align*}
where (\textit{a}) follows from the rule $m_{0}^{(t)} = \tilde{m}_{t-1} =  m_{n}^{(t-1)} $. 

Now taking the sum for $i = 0, 1, \dots, n-1$ we can write  
\begin{align*}
    \frac{1}{n} \sum_{i=0}^{n-1} m_{i+1}^{(t)} =  \beta^n I +  J
\end{align*}
where
\begin{align*}
    I = \frac{1}{n} \sum_{i=0}^{n-1} m_{i+1}^{(t-1)}, 
    J = \frac{1-\beta}{n} \sum_{i=0}^{n-1} \Big(\beta^{n-1} g_{i+1}^{(t-1)} + \dots + \beta^{i+1} g_{n-1}^{(t-1)} + \beta^i g_{0}^{(t)} + \dots  + g_{i}^{(t)}  \Big).
\end{align*}

Now we consider the term $J$.
\begin{align*}
    J &=   \frac{1 - \beta}{n} \sum_{i=0}^{n-1} \Big(\beta^{n-1} g_{i+1}^{(t-1)} + \dots + \beta^{i+1} g_{n-1}^{(t-1)} + \beta^i g_{0}^{(t)} + \dots +  \beta g_{i-1}^{(t)} + g_{i}^{(t)} \Big)\\
    &=  \ \frac{1-\beta}{n}  \Big(\beta^{n-1} g_{1}^{(t-1)} + \beta^{n-2} g_{2}^{(t-1)}
    \dots + \beta^{1} g_{n-1}^{(t-1)} + g_{0}^{(t)} \Big) + \dots\\
    & \quad + \frac{1-\beta}{n}  \Big(\beta^{n-1} g_{i+1}^{(t-1)} 
    + \beta^{n-2} g_{i+2}^{(t-1)}
    + \dots + \beta^{i+1} g_{n-1}^{(t-1)} + \beta^i g_{0}^{(t)}  \dots +  \beta g_{i-1}^{(t)} + g_{i}^{(t)} \Big) + \dots \\
    & \quad +\frac{1-\beta}{n}  \Big( \beta^{n-1} g_{0}^{(t)} + 
    \beta^{n-2} g_{1}^{(t)}
    \dots +  \beta g_{n-2}^{(t)} + g_{n-1}^{(t)} \Big) 
    %
    % &=  \frac{1-\beta}{n}  \Big(\beta^{n-1} g_{1}^{(t-1)} + \beta^{n-2} g_{1}^{(t)} 
    % \dots + \beta g_{1}^{(t)} + g_{1}^{(t)} \Big) + \dots\\
    % &+\frac{1-\beta}{n}  \Big(\beta^{n-1} g_{i+1}^{(t-1)} 
    % + \beta^{n-2} g_{i+1}^{(t-1)}
    % + \dots + \beta^{n-i-1} g_{i+1}^{(t-1)} + \beta^{n-i} g_{i+1}^{(t)} + \dots +  \beta g_{i+1}^{(t)} + g_{i+1}^{(t)} \Big) +
    % \dots\\
    % &+\frac{1-\beta}{n}  \Big( \beta^{n-1} g_{0}^{(t)} + 
    % \beta^{n-2} g_{0}^{(t)}
    % \dots +  \beta g_{0}^{(t)} + g_{0}^{(t)} \Big) 
    %
\end{align*}
% \textcolor{blue}{with a note that the permutation is the same for every epoch}, we get the following result: 
% \begin{align*}
%     J &= \frac{1-\beta}{n} \sum_{i=1}^{n-1} (\beta^{n-1} + \dots + \beta^{n-i}) g_{i}^{(t-1)} 
%     + \frac{1-\beta}{n} \sum_{i=0}^{n-1} (\beta^{n-i-1} + \dots + \beta^{0}) g_{i}^{(t)}
% \end{align*}
Reordering the terms $g_{i}^{(t)}$ and $g_{i}^{(t-1)}$ with a note that $\sum_{j=n}^{n-1} \beta^{j} = 0$ by convention, we get 
\begin{align*}
    J &= \frac{1-\beta}{n} \sum_{i=1}^{n-1} \left( \sum_{j=n-i}^{n-1} \beta^{j} \right) g_{i}^{(t-1)} 
    + \frac{1-\beta}{n} \sum_{i=0}^{n-1} \left( \sum_{j=0}^{n-i-1} \beta^{j} \right) g_{i}^{(t)} \\
    & = \frac{1-\beta}{n} \sum_{i=0}^{n-1} \left[  \left( \sum_{j=n-i}^{n-1} \beta^{j} \right) g_{i}^{(t-1)} +  \left( \sum_{j=0}^{n-i-1} \beta^{j} \right) g_{i}^{(t)}  \right]. 
\end{align*}


% \begin{align*}
%     J &= \frac{1-\beta}{n} \sum_{i=0}^{n-1} (\beta^{n-1} + \dots + \beta^{n-i-1}) g_{i+1}^{(t-1)} 
%     + \frac{1-\beta}{n} \sum_{i=0}^{n-1} (\beta^{n-i} + \dots + \beta^{0}) g_{i+1}^{(t)}\\
%     &= \frac{1-\beta}{n} \sum_{i=0}^{n-1} \left((\beta^{n-1} + \dots + \beta^{n-i-1}) g_{i+1}^{(t-1)} 
%     +  (\beta^{n-i} + \dots + \beta^{0}) g_{i+1}^{(t)} \right)
% \end{align*}
Now applying this formula into the previous sum, we obtain the result of Lemma~\ref{lem_momentum_formula}. 
\end{proof}

\section*{Proof of Theorem~\ref{thm_momentum}}

% \begin{thm}\label{thm_momentum}
% Let $\{w_i^{(t)}\}$ be the sequence generated by Algorithm \ref{sgd_momentum_shuffling} with $\eta_i^{(t)} = \frac{\eta_t}{n}$ and $0 < \eta_t \leq \frac{1}{L}$ for every $t = 1, 2, \dots, T$.
% Then, under Assumption \ref{ass_lower_bound}, \ref{ass_smooth}, and \ref{ass_bounded_gradient}, we have: 
%  \begin{align*}
%     \mathbb{E}\big[\| \nabla F( \hat{w}_T )  \|^2 \big] \leq    \frac{2 [F( \tilde{w}_{1} ) - F_*] + \eta_1 \norms{ \nabla F( \tilde{w}_{0} ) }^2 } {\big(\sum_{t=1}^T \eta_t \big)(1 - \beta^n)}   + \frac{4\beta^n G^2}{1 - \beta^n}    +   L^2 G^2  \frac{\sum_{t=1}^T \xi_t^3}{\sum_{t=1}^T \eta_t}.
%     \tagthis \label{eq_thm_momentum}
% \end{align*}
% where $\xi_t = \max (\eta_t, \eta_{t-1})$ for $t \geq 2$ and $\xi_1 = \eta_1$.
% \end{thm}
\begin{proof}
Since $F$ is $L$-smooth,  for $t\geq 2$, we can derive 
\begin{align*}
    F( w_0^{(t+1)} )  & \overset{\eqref{eq:Lsmooth}}{\leq} F( w_0^{(t)} ) + \nabla F( w_0^{(t)} )^{\top}(w_0^{(t+1)} - w_0^{(t)}) + \frac{L}{2}\norms{w_0^{(t+1)} - w_0^{(t)}}^2  \\
    %
    &\overset{\tiny\eqref{update_momentum_epoch}}{=} F( w_0^{(t)} ) - \eta_t \nabla F( w_0^{(t)} )^\top \left( \frac{1}{n} \sum_{i=0}^{n-1} m_{i+1}^{(t)} \right) + \frac{L \eta_t^{2}}{2} \Big\Vert \frac{1}{n}\sum_{i=0}^{n-1} m_{i+1}^{(t)} \Big\Vert^2  \\
    %
    &\overset{\tiny\eqref{eq_formula_sum}}{=} F( w_0^{(t)} ) - \eta_t \nabla F( w_0^{(t)} )^\top \left( \beta^n I +  J \right) + \frac{L \eta_t^{2}}{2} \Big\Vert \beta^n I +  J \Big\Vert^2  \\
    %
    &\overset{(a)}{\leq} F( w_0^{(t)} ) - \eta_t  \beta^n \nabla F( w_0^{(t)} )^\top  I  - \eta_t \nabla F( w_0^{(t)} )^\top   J  + \frac{L \eta_t^{2}}{2} \beta^n \norms{I}^2 +  \frac{L \eta_t^{2}}{2(1-\beta^n)} \norms{J}^2  \\
    %
    & \overset{(b)}{\leq} F( w_0^{(t)} ) + \eta_t  \beta^n G^2  - \eta_t \nabla F( w_0^{(t)} )^\top   J  +  \frac{L \eta_t^{2}}{2} \beta^n G^2 +  \frac{L \eta_t^{2}}{2(1-\beta^n)} \norms{J}^2  \\
    %
    & \overset{(c)}{\leq} F( w_0^{(t)} )  + 2 \eta_t  \beta^n G^2  - \eta_t \nabla F( w_0^{(t)} )^\top   J   +  \frac{L \eta_t^{2}}{2(1-\beta^n)}  \norms{J}^2    
\end{align*}
where (\textit{a}) comes from the convexity of squared norm: $\norms{\beta^n I +  J}^2 \leq \beta^n \norms{I}^2 +  (1-\beta^n)  \Big\Vert \frac{J}{1-\beta^n} \Big\Vert ^2 $, (\textit{b}) is from the inequalities $\| F( w_0^{(t)} ) \| \leq G$ and $\norms{I} \leq G$  noted in Lemma~\ref{lem_bounded_momentum}, and (\textit{c}) follows from the fact that $L \eta_t \leq 1$.

Now we focus on  the term $\nabla F( w_0^{(t)} )^\top   J$: 
\begin{align*}
    F( w_0^{(t+1)} ) &\leq F( w_0^{(t)} )  + 2 \eta_t  \beta^n G^2  - \eta_t \nabla F( w_0^{(t)} )^\top   J  + \frac{L \eta_t^{2}}{2(1-\beta^n)}  \norms{J}^2 \\
    %
    &= F( w_0^{(t)} )  + 2 \eta_t  \beta^n G^2 - \frac{\eta_t}{1 - \beta^n} (1-\beta^n)\nabla F( w_0^{(t)} )^\top   J   + \frac{L \eta_t^{2}}{2(1-\beta^n)}  \norms{J}^2 \\ 
    %
    &\overset{(d)}{=} F( w_0^{(t)} )  + 2 \eta_t  \beta^n G^2 + \frac{\eta_t}{2(1 - \beta^n)} \Big \Vert (1-\beta^n)\nabla F( w_0^{(t)} ) -   J \Big \Vert^2 \\
    & \quad - \frac{\eta_t}{2(1 - \beta^n)} \Big \Vert (1-\beta^n)\nabla F( w_0^{(t)} )  \Big \Vert^2 
    - \frac{\eta_t}{2(1 - \beta^n)} \norms{J}^2
    + \frac{L \eta_t^{2}}{2(1-\beta^n)}  \norms{J}^2 \\
    %
    &\overset{(e)}{\leq} F( w_0^{(t)} )  + 2 \eta_t  \beta^n G^2 +   \frac{\eta_t}{2(1 - \beta^n)} K
    - \frac{\eta_t(1 - \beta^n)}{2} \Big \Vert \nabla F( w_0^{(t)} )  \Big \Vert^2, \tagthis \label{eq_key_thm_01}
    % & \text{~where~} K = \Big \Vert (1-\beta^n)\nabla F( w_0^{(t)} ) -   J \Big \Vert^2. 
\end{align*}
where $K = \Big \Vert (1-\beta^n)\nabla F( w_0^{(t)} ) -   J \Big \Vert^2$.

In the argument above (\textit{d}) follows from $u^{\top}v = \frac{1}{2}(\norms{u}^2 + \norms{v}^2 - \norms{u - v}^2)$, and  (\textit{e}) comes from the fact that $\eta_t \leq \frac{1}{L}.$ % \textcolor{blue}{\textbf{magic!!!}}

Note that $(1-\beta^n) = (1- \beta) \sum_{j=0}^{n-1}\beta^{j}$ and $\nabla F( w_0^{(t)} ) = \frac{1}{n} \sum_{i=0}^{n-1} \nabla f ( w_{0}^{(t)} ; \sigma^{(t)} ( i + 1 ) )$, we can rewrite that:

\begin{align*}
    (1-\beta^n)\nabla F( w_0^{(t)} ) &= \frac{1-\beta}{n} \sum_{i=0}^{n-1} \left[ \left( \sum_{j=0}^{n-1}\beta^{j} \right) \nabla f ( w_{0}^{(t)} ; \sigma^{(t)} ( i + 1 ) \right]
\end{align*} 

% \begin{align*}
%     (1-\beta^n)\nabla F( w_0^{(t)} ) &= \frac{1-\beta}{n} \sum_{i=0}^{n-1} (\beta^{n-1} + \dots + \beta^{n-i-1} + \beta^{n-i} + \dots + \beta^{0}) \nabla f ( w_{0}^{(t)} ; \sigma^{(t)} ( i + 1 ) 
% \end{align*}
Also recall from Lemma~\ref{lem_momentum_formula} that: \begin{align*}
    J = \frac{1-\beta}{n} \sum_{i=0}^{n-1} \left[  \left( \sum_{j=n-i}^{n-1} \beta^{j} \right) g_{i}^{(t-1)} +  \left( \sum_{j=0}^{n-i-1} \beta^{j} \right) g_{i}^{(t)}  \right]
\end{align*}

% \begin{align*}
%     \qquad \qquad \quad J &= \frac{1-\beta}{n} \sum_{i=0}^{n-1} \left((\beta^{n-1} + \dots + \beta^{n-i-1}) g_{i+1}^{(t-1)} 
%     +  (\beta^{n-i} + \dots + \beta^{0}) g_{i+1}^{(t)} \right)
% \end{align*}
Note that  
\begin{align*}
    h_{i}^{(t)} &= g_{i}^{(t)} - \nabla f ( w_{0}^{(t)} ; \sigma^{(t)} ( i + 1 ) ) \\
    k_{i}^{(t-1)} &= g_{i}^{(t-1)} - \nabla f ( w_{0}^{(t)} ; \sigma^{(t)} ( i + 1 ) ) 
\end{align*}
Now we have the following term 
\begin{align*}
    K &= \Big \Vert (1-\beta^n)\nabla F( w_0^{(t)} ) -   J \Big \Vert^2 \\
    &= \Big \Vert \frac{1-\beta}{n} \sum_{i=0}^{n-1} \left[  \left( \sum_{j=n-i}^{n-1} \beta^{j} \right) k_{i}^{(t-1)} +  \left( \sum_{j=0}^{n-i-1} \beta^{j} \right) h_{i}^{(t)}  \right] \Big \Vert ^2\\
    &\leq \frac{(1-\beta)^2}{n} \sum_{i=0}^{n-1} \Big \Vert  \left( \sum_{j=n-i}^{n-1} \beta^{j} \right) k_{i}^{(t-1)} +  \left( \sum_{j=0}^{n-i-1} \beta^{j} \right) h_{i}^{(t)}  \Big \Vert ^2\\
    &\leq \frac{(1-\beta)^2}{n} \left(\sum_{j=0}^{n-1}\beta^{j} \right)^2  \sum_{i=0}^{n-1} \Big \Vert \frac{\sum_{j=n-i}^{n-1} \beta^{j}}{\sum_{j=0}^{n-1}\beta^{j}}  k_{i}^{(t-1)} + \frac{\sum_{j=0}^{n-i-1} \beta^{j}}{\sum_{j=0}^{n-1}\beta^{j}}   h_{i}^{(t)}  \Big \Vert ^2\\
    %&= \frac{(1-\beta)^2}{n^2} \Big \Vert  \sum_{i=0}^{n-1} \left[  \left( \sum_{j=n-i}^{n-1} \beta^{j} \right) k_{i}^{(t-1)} +  \left( \sum_{j=0}^{n-i-1} \beta^{j} \right) h_{i}^{(t)}  \right] \Big \Vert ^2\\
    & \overset{(f)}{\leq} \frac{(1-\beta)^2}{n} \left(\sum_{j=0}^{n-1}\beta^{j} \right)^2 \sum_{i=0}^{n-1}   \left [ \frac{\sum_{j=n-i}^{n-1} \beta^{j}}{\sum_{j=0}^{n-1}\beta^{j}}   \norms{k_{i}^{(t-1)}} ^2
    + \frac{\sum_{j=0}^{n-i-1} \beta^{j}}{\sum_{j=0}^{n-1}\beta^{j}}  \norms{h_{i}^{(t)}}^2 \right] \\
    &\leq \frac{(1-\beta)^2}{n} \left(\sum_{j=0}^{n-1}\beta^{j} \right)^2 \sum_{i=0}^{n-1} \max \Big( \norms{k_{i}^{(t-1)}} ^2; \norms{h_{i}^{(t)}}^2 \Big) \\
    &\leq \frac{(1-\beta^n)^2}{n}  \sum_{i=0}^{n-1} \max \Big( \norms{k_{i}^{(t-1)}} ^2; \norms{h_{i}^{(t)}}^2 \Big) 
    \overset{(g)}{\leq}  (1-\beta^n)^2 L^2 G^2 \xi_t^2
\end{align*}
where (\textit{f}) is from the convexity for squared norm function, and (\textit{g}) follows from Lemma~\ref{lem_bounded_02} with $\xi_t^2 = \max (\eta_t^2; \eta_{t-1}^2)$ for $t\geq 2$.

Applying this expression to \eqref{eq_key_thm_01} for $t\geq 2$, we obtain that: 
\begin{align*}
    F( w_0^{(t+1)} ) 
    \leq F( w_0^{(t)} )  + 2 \eta_t  \beta^n G^2 +   \frac{\eta_t (1 - \beta^n)}{2}  L^2 G^2 \xi_t^2
    - \frac{\eta_t(1 - \beta^n)}{2} \Big \Vert \nabla F( w_0^{(t)} )  \Big \Vert^2.  
\end{align*}
Note that $\tilde{w}_{t-1} = w_0^{(t)}$ and $\tilde{w}_{t} = w_0^{(t+1)}$, this leads to  
% \begin{align*}
%   \frac{\eta_t(1 - \beta^n)}{2} \Big \Vert \nabla F( w_0^{(t)} )  \Big \Vert^2
%     \leq F( w_0^{(t)} ) -  F( w_0^{(t+1)} )   + 2 \eta_t  \beta^n G^2 +   \frac{\eta_t (1 - \beta^n)}{2}  L^2 G^2 \xi_t^2
%        
% \end{align*}
\begin{align*}
     \eta_t \Big \Vert \nabla F( \tilde{w}_{t-1} )  \Big \Vert^2 \leq  \frac{2 [F( \tilde{w}_{t-1} ) - F( \tilde{w}_{t})]} {(1 - \beta^n)}   + \frac{4\beta^n G^2}{1 - \beta^n} \eta_t  +   L^2 G^2 \xi_t^3, \ \  t \geq 2.
\end{align*}

For the convenience of our analysis, we denote that $\xi_1 = \eta_1$ and derive the following statement for $t=1$: 
\begin{align*}
     \eta_t \Big \Vert \nabla F( \tilde{w}_{t-1} )  \Big \Vert^2 \leq  \frac{\eta_t \norms{ \nabla F( \tilde{w}_{t-1} ) }^2 }{1 - \beta^n}   + \frac{4\beta^n G^2}{1 - \beta^n} \eta_t  +   L^2 G^2 \xi_t^3.
\end{align*} 

Summing the previous statements for $t = 1, 2, \dots, T$ we obtain that 
\begin{align*}
     \sum_{t=1}^T \left(\eta_t \Big \Vert \nabla F( \tilde{w}_{t-1} )  \Big \Vert^2  \right) \leq   \frac{2 [F( \tilde{w}_{1} ) - F_* ] + \eta_1 \norms{ \nabla F( \tilde{w}_{0} ) }^2 } {(1 - \beta^n)}   + \frac{4\beta^n G^2}{1 - \beta^n}  \sum_{t=1}^T \eta_t  +   L^2 G^2  \sum_{t=1}^T \xi_t^3.
\end{align*}


Hence, dividing by $\sum_{t=1}^T \eta_t$ to both sides, the desired result follows immediately.

% \begin{align*}
%     \frac{1}{\sum_{t=1}^T \eta_t} \sum_{t=1}^T \left(\eta_t \Big \Vert \nabla F( \tilde{w}_{t-1} )  \Big \Vert^2  \right) \leq    \frac{2 [F( \tilde{w}_{1} ) - F_*] + \eta_1 \norms{ \nabla F( \tilde{w}_{0} ) }^2 } {\big(\sum_{t=2}^T \eta_t \big)(1 - \beta^n)}   + \frac{4\beta^n G^2}{1 - \beta^n}    +   L^2 G^2  \frac{\sum_{t=2}^T \xi_t^3}{\sum_{t=2}^T \eta_t}.
%       
% \end{align*}
%\trang{Note: Let $\beta = (\frac{\delta}{T^{2/3}})^{1/n} < 1$ for some $ \delta > 0$}
\end{proof}
